Evidentiality-aware Retrieval for Overcoming Abstractiveness in Open-Domain Question Answering

The long-standing goal of dense retrievers in abtractive open-domain question answering (ODQA) tasks is to learn to capture evidence passages among relevant passages for any given query, such that the reader produce factually correct outputs from evidence passages. One of the key challenge is the insufficient amount of training data with the supervision of the answerability of the passages. Recent studies rely on iterative pipelines to annotate answerability using signals from the reader, but their high computational costs hamper practical applications. In this paper, we instead focus on a data-centric approach and propose Evidentiality-Aware Dense Passage Retrieval (EADPR), which leverages synthetic distractor samples to learn to discriminate evidence passages from distractors. We conduct extensive experiments to validate the effectiveness of our proposed method on multiple abstractive ODQA tasks.

==> figure_latex/4_method/counterfactual_overview.tex <==
\begin{figure*}[t]
    
    \centering
    % \hspace*{\fill}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/pseudo_evi_annotation.pdf}
        \caption{Pseudo-evidentiality annotation}
        \label{fig:masking_strategy}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{figure/learning strategy.pdf}
        \caption{Counterfactual pivots in the embedding space}
        \label{fig:pivot-concept}
    \end{subfigure}
    
    \caption{ Illustration of (a) pseudo-evidentiality annotation and (b) AADPR learning strategy. }
    \label{fig:cf_overview}
\end{figure*}

==> figure_latex/analysis_aar.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/similarity_comparison.pdf}
        \caption{Similarity Scores}
        \label{similarity_comparison}
    \end{subfigure}
    \begin{subfigure}[b]{0.26\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/score_distribution.pdf}
        \caption{Distribution of similarity}
        \label{similarity_distribution}
    \end{subfigure}
    \caption{(a) Similarity scores between queries and positive passages or counterfactual passages in DPR and DPR+PiCL. (b) Distributions of score differences $\langle q,p^+ \rangle - \langle q,p^* \rangle$ drawn from DPR and DPR+PiCL.}
    \label{fig:analysis_section2}
\end{figure}

%\caption{Similarity scores between queries and positive passages     or counterfactual passages in DPR and DPR+PiCL.}

%\captionof{figure}{Retrieval performance of DPR and DPR+PiCL on varying the numbers of negatives.}

==> figure_latex/analysis_rel.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{figure/analysis_number_of_negatives.pdf}
    \caption{Retrieval performance of DPR and DPR+PiCL on varying the numbers of negatives. 
    }
    \label{fig:analysis-neg-num}
\end{figure}

%\caption{Similarity scores between queries and positive passages     or counterfactual passages in DPR and DPR+PiCL.}

%\captionof{figure}{Retrieval performance of DPR and DPR+PiCL on varying the numbers of negatives.}

==> figure_latex/learning_strategy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/learning strategy.pdf}
    \caption{Illustration of our counterfactual learning strategy.}
    \label{fig:learning_strategy}
\end{figure}


==> figure_latex/masking_strategy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/sampling strategy.pdf}
    % {figure/sample_pivot.png}
    \caption{Illustration of the counterfactual samples as pivots in the embedding space.}
    \label{fig:masking_strategy}
\end{figure}
%The blue and white boxed texts represent the gold answer and the answer sentence $a$, respectively.

==> figure_latex/pivot_concept.tex <==

%\begin{figure*}[!htd]
\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/pivot_concept.pdf}
         \caption{Conceptualization of counterfactual pivots.}
         \label{fig:pivot-concept}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/SBERT_psg_sim_half.pdf}
         \caption{{Similarity scores between queries and various type of passages obtained by SBERT~\citep{reimers2019sbert}.}}
         \label{fig:pivot-sim}
     \end{subfigure}
     \hfill
    \caption{\textbf{(a)}~Illustration of the counterfactual samples as pivots in the embedding space. {\textbf{(b)}~Comparison of cosine similarity scores between queries and passages with various types (\eg, positive, counterfactal, BM25 hard negative, and random).}}
    \label{figure:pivot-explain}
\end{figure}
    

==> figure_latex/pivot_explanation.tex <==
%\begin{figure*}[!htd]
\begin{figure}[t]
    \centering
    \begin{center}
    \includegraphics[width=0.85\linewidth]{figure/pivot_concept.pdf}
    \end{center}
    \caption{Illustration of the counterfactual samples as pivots in the embedding space.}
    \label{figure:pivot-explain}
\end{figure}

==> figure_latex/qtype_analysis_1col.tex <==
\begin{figure}[t]

    \centering
    \begin{subfigure}[b]{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/question_types_AA Score small.png}
        \caption{Answerability Awareness}
        \label{fig:qtype-aa}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/question_types_Top-5 Accuracy small.png}
        \caption{Retrieval Top-5 Accuracy}
        \label{fig:qtype-top5}
    \end{subfigure}
    % \centering
    % \begin{center}
    %     \includegraphics[width=\linewidth]{figure/question_types.png}
    % \end{center}
    \caption{AA score and retriever top-5 accuracy on various question types.}
    \label{fig:qtype}
\end{figure}



==> figure_latex/resource_efficiency.tex <==
\begin{figure}[t]
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/analysis_number_of_negatives.pdf}
        \caption{Number of negatives}
        \label{fig:label_negative}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
            \includegraphics[width=\textwidth]{figure/similarity_comparison.pdf}
            \caption{Similarity scores}
            \label{fig:similarity_comparison}
    \end{subfigure}
    \caption{(a) Retrieval performance of DPR and \our~on varying the numbers of negatives.}
    \label{fig:analysis_section}
\end{figure}

==> figure_latex/robustness_analysis.tex <==
\begin{figure}[t]

    \centering
    \includegraphics[width=\linewidth]{figure/AA_num_neg.png}
    
    \caption{Plot of AA scores of DPR and EADPR.}
    \label{fig:aa_experiment}
\end{figure}


==> figure_latex/robustness_analysis_emnlp.tex <==
\begin{figure}[t]

    \centering
    \includegraphics[width=\linewidth]{figure/AA_num_neg.png}
    
    \caption{Plot of AA scores and the total number of additional negative passages retrieved during model training on Natural Questions.}
    \label{fig:aa_experiment}
\end{figure}


==> figure_latex/sbert.tex <==
%\begin{figure*}[!htd]
\begin{figure}[t]
    \centering
    \begin{center}
    \includegraphics[width=0.9\linewidth]{figure/SBERT_psg_sim_half.pdf}
    \end{center}
    \caption{Comparison of cosine similarity scores between queries and passages of various types (\eg, positive, counterfactual, BM25 hard negative, and random).}
    \label{fig:sbert-sim}
\end{figure}

==> figure_latex/score_distribution.tex <==
\begin{figure}[t]
    \centering
    \begin{center}
        \includegraphics[width=0.9\linewidth]{figure/distribution.jpg}
    \end{center}
    \caption{Relevance score difference between positive and counterfactual passages from DPR and AADPR.}
    \label{fig:similarity_comparison_acl}
\end{figure}

==> figure_latex/score_histogram.tex <==


\begin{figure}[t]
    %\vspace{-12pt}
    \begin{center}
        \includegraphics[width=0.6\linewidth]{figure/score_distribution.pdf}
    \end{center}
    \caption{Distributions of score differences $\langle q,p^+ \rangle - \langle q,p^* \rangle$ drawn from DPR and DPR+PiCL.}
    \label{fig:score_histogram}
\end{figure}



==> figure_latex/sim_score_analysis.tex <==

%\begin{figure*}[!htd]
\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figure/similarity_comparison-3.pdf}
         \caption{Comparison of similarity scores $\langle q,p^+ \rangle$ and $\langle q,p^* \rangle$
    in DPR and DPR+PiCL.}
         \label{fig:sim-compare}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/score_distribution-3.pdf}
         \caption{{Distributions of score differences $\langle q,p^+ \rangle - \langle q,p^* \rangle$ drawn from DPR and DPR+PiCL.}}
         \label{fig:sim-histo}
     \end{subfigure}
     \hfill
    \caption{{Similarity score differences between queries and positive passages or counterfactual passages in DPR and DPR+PiCL.}}
    \label{fig:score-analysis}
\end{figure}
    

==> figure_latex/similarity_comparison.tex <==


\begin{figure}
    % \vspace{-22pt}
    % \centering
    \begin{center}
    \includegraphics[width=0.3\linewidth]{figure/similarity_comparison.pdf}
    \end{center}
    \caption{Similarity scores 
    between queries and positive passages or counterfactual passages in 
    DPR and DPR+PiCL.}
    \label{fig:similarity_comparison}
    % \vspace{-20pt}
\end{figure}



==> tables/ablation_studies_iclr.tex <==


\begin{minipage}{\textwidth}\scriptsize
  \begin{minipage}[b]{0.35\textwidth}
    \centering
    % \includegraphics[width=0.8\linewidth]{figure/example of visualization.pdf}
    \includegraphics[width=0.8\linewidth]{figure/analysis number of negatives.pdf}
    \captionof{figure}{Retrieval performance of DPR and DPR+PiCL on varying the numbers of negatives.}
    \label{fig:label_negative}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.6\textwidth}
    \centering
    \begin{tabular}{l c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{Retriever}}&\multicolumn{4}{c}{\textbf{Natural Questions}}\\
    \cline{2-5}
    & Top-1 & Top-5 & Top-20 & Top-100 \\
\hline
\noalign{\hrule height0.8pt}
     % DPR &29.78&56.15& 68.39 & 81.25 \\
     % DPR &29.78&56.15&74.20&84.40 \\
        DPR &32.08&59.56&76.54&85.73 \\

\hline
     (1) Counterfactual Loss &   &  & & \\
     ~ $\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{cpp}}$ &28.14&56.65&75.12&85.54 \\ 
     ~ $\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{chn}}$ &30.80&58.59&75.98&84.85 \\ 
     ~ $\mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$ &33.35&61.36&77.87&{86.09}\\ 
     % ~ \textbf{$\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$} &\textbf{44.85}&\textbf{68.01}& \textbf{78.78} & {85.71}  \\
     ~ \textbf{$\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$}
     &33.99&61.88&77.7&85.84 \\
 \hline
     (2) Counterfactual Sampling & & & &   \\
     %PiCL$_{\texttt{random}}$ &31.19&59.22& 75.98 & {85.40} \\ 
     ~ {PiCL$_{\texttt{answer}}$} &30.28&57.12& 73.99 & 84.52  \\ 
     ~ {PiCL$_{\texttt{window}}$} &31.50&60.03& {76.40} & {85.18}  \\ 
     ~ {PiCL$_{\texttt{sentence}}$}&33.99&61.88&77.7&85.84 \\ 
     %\hline
     %PiCL$_{\texttt{BM25}}$ & 37.26 & 78.45 & 86.15 \\ 
     %PiCL$_{\texttt{DPR}}$ & - & - & - \\ 
     
     % PiCL$_{\texttt{random}}$ & 75.98 & \textbf{85.4} \\ 
     % \textbf{PiCL$_{\texttt{causal}}$} & \textbf{76.4} & {85.18}  \\ 
     % \hline
     % PiCL$_{\texttt{BM25}}$ & - & \textbf{-} \\ 
     
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 \captionof{table}{Ablation studies on PiCL.}
 \vspace{8pt}
 \label{tables:ablation_studies}
    \end{minipage}
  \end{minipage}
 

==> tables/ablation_studies_loss_backup.tex <==


\begin{table}[t]\small
\centering
\renewcommand{\arraystretch}{1.15} %1.15
\begin{tabular}{l c c c c}
\hline
    \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{Retriever}}&\multicolumn{4}{c}{\textbf{Natural Questions}}\\
    \cline{2-5}
    &Top-1 &Top-5 &Top-20 &Top-100\\
\hline
\noalign{\hrule height0.8pt}
     $\mathcal{L}_{\texttt{dpr}}$ 
     % &32.08&59.56&76.54&85.73 \\
     &31.77&58.12&74.76&84.07 \\
\hline
     %\our~& & &  &  \\
     ~ $+ \mathcal{L}_{\texttt{cpp}}$ 
     % &28.14&56.65&75.12&85.54 \\ 
     &28.31&55.84&74.57&84.32 \\
     %&36.34&62.66&77.78&85.6 \\
     ~ $+ \mathcal{L}_{\texttt{chn}}$ 
     % &30.80&58.59&75.98&84.85 \\ 
     &32.58&59.25&75.65&84.90 \\
     %&36.9&62.13&76.79&84.99 \\
     %$\mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$ &33.35&61.36&77.87&{86.09} \\ 
     ~ \textbf{$+ \mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$}
     % &33.99&61.88&77.70&85.84 \\
     &35.35& &76.81&85.87 \\
\hline
\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{Ablation studies on the training objective.}

\label{tables:ablation_studies_loss}
\end{table}

==> tables/ablation_studies_negative.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.8\linewidth]{figure/example of visualization.pdf}
    \includegraphics[width=0.8\linewidth]{figure/analysis number of negatives.pdf}
    \captionof{figure}{Retrieval performance of DPR and DPR+PiCL on varying the numbers of negatives.}
    \label{fig:label_negative}
\end{figure}

==> tables/ablation_studies_old.tex <==


\begin{table}[h]
    \centering
    \begin{tabular}{l c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{Retriever}}&\multicolumn{4}{c}{\textbf{Natural Questions}}\\
    \cline{2-5}
    & Top-1 & Top-5 & Top-20 & Top-100 \\
\hline
\noalign{\hrule height0.8pt}
     % DPR &29.78&56.15& 68.39 & 81.25 \\
     % DPR &29.78&56.15&74.20&84.40 \\
        DPR &32.08&59.56&76.54&85.73 \\

\hline
     (1) Counterfactual Loss &   &  & & \\
     ~ $\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{cpp}}$ &28.14&56.65&75.12&85.54 \\ 
     ~ $\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{chn}}$ &30.80&58.59&75.98&84.85 \\ 
     ~ $\mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$ &33.35&61.36&77.87&{86.09}\\ 
     % ~ \textbf{$\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$} &\textbf{44.85}&\textbf{68.01}& \textbf{78.78} & {85.71}  \\
     ~ \textbf{$\mathcal{L}_{\texttt{dpr}} + \mathcal{L}_{\texttt{cpp}} + \mathcal{L}_{\texttt{chn}}$}
     &33.99&61.88&77.7&85.84 \\
 \hline
     (2) Counterfactual Sampling & & & &   \\
     %PiCL$_{\texttt{random}}$ &31.19&59.22& 75.98 & {85.40} \\ 
     ~ {PiCL$_{\texttt{answer}}$} &30.28&57.12& 73.99 & 84.52  \\ 
     ~ {PiCL$_{\texttt{window}}$} &31.50&60.03& {76.40} & {85.18}  \\ 
     ~ {PiCL$_{\texttt{sentence}}$}&33.99&61.88&77.7&85.84 \\ 
     %\hline
     %PiCL$_{\texttt{BM25}}$ & 37.26 & 78.45 & 86.15 \\ 
     %PiCL$_{\texttt{DPR}}$ & - & - & - \\ 
     
     % PiCL$_{\texttt{random}}$ & 75.98 & \textbf{85.4} \\ 
     % \textbf{PiCL$_{\texttt{causal}}$} & \textbf{76.4} & {85.18}  \\ 
     % \hline
     % PiCL$_{\texttt{BM25}}$ & - & \textbf{-} \\ 
     
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 \captionof{table}{Ablation studies on PiCL.}
 \vspace{8pt}
 \label{tables:ablation_studies_loss}
\end{table}

==> tables/ablation_studies_sampling.tex <==


\begin{table}[t]\small
\renewcommand{\arraystretch}{1.15} %1.15
\centering

\begin{tabular}{l c c c c }
\hline
    \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{Retriever}}&\multicolumn{4}{c}{\textbf{Natural Questions}}\\
    \cline{2-5}
    &Top-1 &Top-5 &Top-20 &Top-100 \\
\hline
\noalign{\hrule height0.8pt}
     DPR &32.08&59.56&76.54&85.73 \\
\hline
     {\our$_{\text{answer}}$} &30.28&57.12& 73.99 & 84.52  \\ 
     {\our$_{\text{window}}$} &31.50&60.03& {76.40} & {85.18}  \\ 
     \textbf{{\our$_{\text{sentence}}$}}&\textbf{33.99}&\textbf{61.88}&\textbf{77.7}&\textbf{85.84} \\  
\hline
\noalign{\hrule height 0.8pt}
\end{tabular}

\caption{Ablation studies on different counterfactual sampling strategies for \our.}

\label{tables:ablation_studies_sampling}
\end{table}

==> tables/dataset_length_analysis.tex <==
\begin{table*}[!ht]
\begin{tabular}{l c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \textbf{dataset}
    & \#N samples & avg(span) &avg(passage) & 15\% of avg(passage) ($\ell$) \\
\hline
\noalign{\hrule height0.8pt}
     NaturalQuestions   & 58880 & 2.31 & 104.89 & 15.73 (16)\\ 
     % NaturalQuestions   & 58812 & 2.31 &104.89  & 15.73 (16)\\ 
     % #N 빼고 나머지 결과는 같음
     SQuAD   & N & N & N & \\ 
     TriviaQA   & N & N & N & \\ 
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}

\caption{The analysis of benchmark datasets. avg($X$) indicates the average number of tokens for a given $X$.}
\label{table:datasetAnalysis}
%PMI-Masking 논문에서는 caption을 아래에 달았음.. %
\end{table*}


==> tables/downstream.tex <==
\begin{table*}[!ht]\small
\renewcommand{\arraystretch}{1.2} %1.5
\centering

\begin{tabular}{c c c c c c  }
\hline
\noalign{\hrule height 0.8pt}

\multirow{2}{*}{\textbf{Reader}}&\multirow{2}{*}{\textbf{Retriever}}&NQ&TQA&T-REx \\
% \cmidrule(lr){4-5}\cmidrule(lr){6-7}
\cmidrule{3-5}
&&Exact Match&Exact Match&F1  \\

\hline
\noalign{\hrule height 0.8pt}

%\midrule

% \noalign{\hrule height0.8pt}

% \multirow{2}{*}{{127}}&\multirow{2}{*}{{DPR reader}}&DPR&{31.83}
%  &{36.87}&{37.45}
% \\
% &&{\our}&{34.52} (+2.69)&{{38.31} (+1.44)}&{{38.81} (+1.36)}
% \\
% \multirow{4}{*}{{127+128}}&\multirow{2}{*}{{DPR reader}}&DPR&{68.56 $\mapsto$ 38.48}
%  &{79.7 $\mapsto$ 39.81}&{86.34 $\mapsto$ 39.81}
% \\
% \multirow{4}{*}{{127+128}}&\multirow{2}{*}{{DPR reader}}&DPR&{38.48}
%  &{39.81}&{39.81}
% \\
% &&{\our} &{{38.12} (-0.36) }&{{38.70} (-1.11)}&{{38.70} (+-)}
% \\
% \cline{2-9}
% \multirow{4}{*}{{127+128}}&\multirow{2}{*}{{DPR reader}}&DPR&{38.48}
%  &{39.81}&{39.81}
% \\
% &&{\our} &{{38.67} (+0.19) }&{{38.70} (-1.11)}&{{38.70} (+-)}
% \\
\multirow{2}{*}{{FiD$_{\text{base}}$ (T5)}}&DPR&{45.37}&-&- \\
&{\our}&{\textbf{47.65} (+2.28)}&-&-\\
% &&{\our}&{\textbf{39.72} (+1.41) }&{\textbf{43.68} (+0.55)}&{\textbf{46.51} (+1.14)} % clean title

\hline
\multirow{2}{*}{ChatGPT}&DPR&{-}&{-}&{-} \\
&{\our}&{-}&{-}&{-} \\ % org
% &&{\our}&{{34.16} (+2.17) }&{{41.83} (+2.72)}&{{46.20} (+2.38)} %clean title
\hline
    
    
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
\caption{Downstream performance of retriever-reader pipelines on extractive tasks. For retrievers, we choose the best-performing DPR and EADPR models from Table~\ref{tab:main_retrieval}. For readers, we consider the 
\#N : number of negative samples used to train the retriever, computed as in-batch negatives (+ BM25 negatives), Top-$k$: top-$k$ retrieved passages for reader inference. Note that we reuse the checkpoints of DPR reader and FiD$_{\text{base}}$ (\ie{ T5-base implementation of FiD}) from \citet{karpukhin2020dpr} and \citet{izacard2021distilling}. Best scores are in \textbf{Bold}.}

\label{table:reader}
\end{table*}


%Note that we reuse the \textcolor{blue}{DPR reader and Fusion-in-Decoder base (FiD$_{\text{base}}$)} models from \citet{karpukhin2020dpr} and \citet{izacard2021distilling}, switching retrievers to obtain EM score.

==> tables/epoch.tex <==
\begin{table*}[!ht]\small

\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    {\textbf{Retriever}}&\multicolumn{4}{c}{\textbf{NaturalQuestions}}\\
    - epoch&top-1&top-5&top-20 & top-100 \\
\hline
\noalign{\hrule height0.8pt}
\textbf{DPR$_{\text{inbatch}}$ } \\
- 25 &29.78&56.15&74.2&84.4 \\
- 40 \\
\hline
     \textbf{PiCL$_{\text{inbatch}}$}\\
     - 23 (best) &29.5&57.53&74.85&84.43\\
     - 25&29.47&56.79&74.93&84.57\\
     - 40&26.84&53.3&70.86&82.66\\
     
     
     
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 
\caption{} 
\label{table:epoch}

\end{table*}




==> tables/ernie.tex <==
\begin{table}[t]\small
\renewcommand{\arraystretch}{1.15} %1.15
\centering

\begin{tabular}{l c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \textbf{\our} &\multicolumn{3}{c}{\textbf{NaturalQuestions}}\\
    \cline{2-4}
    ~~- \textbf{PLM}&Top-1&Top-20&Top-100 \\
\hline
\noalign{\hrule height0.8pt}
    % \multicolumn{1}{l}{\our}\\
    %{BERT$_{\text{base}}$}&47+48&45.38&66.79&78.53\\ % &85.04\\
    %{ERNIE$_{\text{base}}$}&47+48&47.29&68.92&79.53\\ % &85.98\\
    ~~~- {BERT$_{\text{base}}$}&45.38&78.53&85.04\\
% \hline
    ~~~-  {ERNIE$_{\text{base}}$}&49.50 &80.06 &86.23 \\
    ~~~-  {Contriever}&47.01&80.55&86.64\\
    ~~~-  {Condenser}&\textbf{50.06}&\textbf{80.80}&\textbf{86.81}\\
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}

 \caption{Retrieval performance of \our~with different PLMs (i.e., ERNIE, Contriever, Condenser) for retriever initialization. }
 
\label{table:ernie}

\end{table}




==> tables/ernie_iclr.tex <==
\begin{table*}[t]\small

\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{PLM}}&\multirow{2}{*}{\textbf{\# N}}&\multicolumn{4}{c}{\textbf{NaturalQuestions}}\\
    \cline{3-6}
    &&Top-1&Top-5&Top-20 & Top-100 \\
\hline
\noalign{\hrule height0.8pt}
 
%      DPR & \multirow{3}{*}{ERNIE$_{\text{base}}$}\\
%      - {inbatch} &&29.39&56.34&73.93&84.4 \\
%      - {BM25 hard negative} &&45.87&67.98&\textbf{79.7}&\textbf{86.09} \\
     
% \hline
    {BERT$_{\text{base}}$}&47+48&45.38&66.79&78.53&85.04\\
     {ERNIE$_{\text{base}}$}&47+48&47.29&68.92&79.53&85.98\\
     {ERNIE$_{\text{base}}$}&127+128&\textbf{49.5}&\textbf{69.36}&\textbf{80.06}&\textbf{86.23}\\

\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 \caption{Retrieval performance with using a better PLM (i.e., ERNIE). PLMs: pre-trained LMs used for retriever initialization, \# N: number of negative samples. Best scores are in \textbf{Bold}.}
 
\label{table:ernie}

\end{table*}




==> tables/ernie_save.tex <==
\begin{table*}[t]\small

\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{Retriever}}&\multirow{2}{*}{\textbf{PLM}}&\multicolumn{4}{c}{\textbf{NaturalQuestions}}\\
    \cline{3-6}
    &&Top-1&Top-5&Top-20&Top-100 \\
\hline
\noalign{\hrule height0.8pt}

    %{BERT$_{\text{base}}$}&47+48&45.38&66.79&78.53\\ % &85.04\\
    %{ERNIE$_{\text{base}}$}&47+48&47.29&68.92&79.53\\ % &85.98\\
    DPR+PiCL&{BERT$_{\text{base}}$}&45.38&66.79&78.53&85.04\\
\hline
    DPR+PiCL&{ERNIE$_{\text{base}}$}&49.5 (+4.12)&69.36 (+2.57)&80.06 (+1.53)&86.23 (+1.19)\\
    DPR+PiCL&{Contriever}&47.01 (+1.63)&69.22 (+2.43)&80.55 (+2.02)&86.64 (+1.60)\\
    DPR+PiCL&{coCondenser}&\textbf{50.06 (+4.68)}&\textbf{71.16 (+4.37)}&\textbf{80.80 (+2.27)}&\textbf{86.81 (+1.77)}\\
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 \caption{Retrieval performance of DPR+PiCL with different PLMs (i.e., ERNIE, Contriever, coCondenser). PLMs: pre-trained LMs used for retriever initialization.}
 
\label{table:ernie}

\end{table*}




==> tables/ernie_top5.tex <==
\begin{table}[t]\small
\renewcommand{\arraystretch}{1.5} %1.15
\centering
\begin{tabular}{l c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{PLM}}&\multicolumn{3}{c}{\textbf{NaturalQuestions}}\\
    \cline{2-4}
    &Top-5&Top-20&Top-100 \\
\hline
\noalign{\hrule height0.8pt}
    \multicolumn{1}{l}{DPR+PiCL}\\
    %{BERT$_{\text{base}}$}&47+48&45.38&66.79&78.53\\ % &85.04\\
    %{ERNIE$_{\text{base}}$}&47+48&47.29&68.92&79.53\\ % &85.98\\
    ~~~-{BERT$_{\text{base}}$}&66.79&78.53&85.04\\
% \hline
    ~~~- {ERNIE$_{\text{base}}$}&69.36 &80.06 &86.23 \\
    ~~~- {Contriever}&69.22&80.55&86.64\\
    ~~~- {coCondenser}&\textbf{71.16 }&\textbf{80.80}&\textbf{86.81}\\
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 \caption{Retrieval performance of DPR+PiCL with different PLMs (i.e., ERNIE, Contriever, coCondenser). PLMs: pre-trained LMs used for retriever initialization.}
 
\label{table:ernie}

\end{table}




==> tables/ernie_wide.tex <==
\begin{table*}[t]\small

\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l l l l l}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{PLM}}&\multicolumn{4}{c}{\textbf{NaturalQuestions}}\\
    \cline{2-5}
    &\multicolumn{1}{l}{Top-1}&\multicolumn{1}{l}{Top-5}&\multicolumn{1}{l}{Top-20}&\multicolumn{1}{l}{Top-100} \\
\hline
\noalign{\hrule height0.8pt}

    %{BERT$_{\text{base}}$}&47+48&45.38&66.79&78.53\\ % &85.04\\
    %{ERNIE$_{\text{base}}$}&47+48&47.29&68.92&79.53\\ % &85.98\\
    DPR+PiCL\\
    ~~~- {BERT$_{\text{base}}$}&45.38&66.79&78.53&85.04\\
~~~-{ERNIE$_{\text{base}}$}&49.50 (+4.12)&69.36 (+2.57)&80.06 (+1.53)&86.23 (+1.19)\\
    ~~~-{Contriever}&47.01 (+1.63)&69.22 (+2.43)&80.55 (+2.02)&86.64 (+1.60)\\
    ~~~-{coCondenser}&\textbf{50.06 (+4.68)}&\textbf{71.16 (+4.37)}&\textbf{80.80 (+2.27)}&\textbf{86.81 (+1.77)}\\
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 \caption{Retrieval performance of DPR+PiCL with different PLMs (i.e., ERNIE, Contriever, coCondenser). PLMs: pre-trained LMs used for retriever initialization.}
 
\label{table:ernie}

\end{table*}




==> tables/knowledge_distillation.tex <==
\begin{table*}[!ht]\small
% \begin{table}
\caption{Reader distilled model comparison. $^\dag$ represents the reported result from the related paper. FiD$_{16}$ denotes the reproduced setting on our environments, using a distribution of 16 passages per one query, rather than 100 passages.
}
\renewcommand{\arraystretch}{1.5} %1.15
\centering
% \begin{tabular}{l c c | c c}
\begin{tabular}{l c c }
\hline
 \noalign{\hrule height 0.8pt}
 \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{2}{c}{\textbf{NaturalQuestions}}\\
 % & \multicolumn{2}{c}{\textbf{Perturbed NaturalQuestions}} \\
     &top-20 & top-100 \\
     % & top-20 & top-100 \\
\hline


\noalign{\hrule height0.8pt}
     DPR$^\dag$ & 68.39 & 81.25 \\
     {DPR+PiCL} & 77.17 & 85.9 \\ 
     \hline
     BERT + FiD (Reader-distilled) $^\dag$ & 68.8 & 79.5 \\  
     DPR + FiD (Reader-distilled) $^\dag$ & 84.3 & 89.3 \\  
     BERT + FiD$_{16}$ (Reader-distilled) & - & - \\  
     DPR + FiD$_{16}$ (Reader-distilled) & - & - \\
     PiCL + FiD$_{16}$ (Reader-distilled) & - & -  \\ 
\hline

 \noalign{\hrule height 0.8pt}
 \end{tabular}
 
\label{table:distillation}
\end{table*}

==> tables/l1_lambda.tex <==
\begin{table*}[!ht]\small

\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l c | c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    {\textbf{Retriever}}&\multirow{2}{*}{Negative}&\multicolumn{4}{c}{\textbf{NaturalQuestions}}\\
    - $\lambda$ &&top-1&top-5&top-20 & top-100 \\
\hline
\noalign{\hrule height0.8pt}
DPR &random&32.08&59.56&76.54&85.73\\
\hline
     {PiCL}\\
     - $\lambda$ = 0.0 &random&30.28&57.12&73.99&84.52\\
     - $\lambda$ = 0.2 &random&31.63&59.34&76.18&85.29\\
     % - $\lambda$ = 1.0 &random&33.99&61.88&77.7&85.84\\
     
     
     
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 
\caption{} 
\label{table:l1_lambda}

\end{table*}




==> tables/main_resul_no_top5t.tex <==
\begin{table*}[t]\small
%\begin{table}
%\renewcommand{\arraystretch}{1.5} %1.15
\centering

 
\begin{tabular}{l c c c| c c c c| c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{4}{c}{\textbf{Natural Questions}}&\multicolumn{4}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-8}\cmidrule{9-12}
     &PLM &\#N&Hard Neg&Top-1 & Top-5 &Top-20 & Top-100&Top-1 &Top-20 & Top-100&MAP@100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 59.1 & 73.7 & - & 66.9 & 76.7&-\\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127 & - & - & 55.8 & 73.0 & 83.1 & -  & 79.4 & 85.0& -  \\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 81.9 & 87.5& - & 80.3 & 85.3& -  \\
     RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0& - & - & - & -  \\
     RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5& - & -&-& -  \\
     %coCondenser$^\dag$&BERT$_{\text{base}}$&-&-&-&75.8&84.3&89.0\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &31.77&58.12&74.76&84.07&38.72&74.71&82.29&27.78\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &46.62&68.56&79.70&86.34&54.26&79.66&85.34&31.36\\
     %DPR$^*$&BERT$_{\text{base}}$&127+128&DPR&52.69& 72.63&81.44&87.48\\
     
\hline 
 
     {DPR+PiCL}&BERT$_{\text{base}}$& 127&-&32.69&60.39&76.73&85.48&43.02&74.67&82.24&37.93\\ 
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&BM25&\underline{47.81}&\underline{69.25}&\underline{79.92}&\textbf{87.12}&\underline{56.93}&\underline{80.46}&\textbf{85.72}&\textbf{39.4}\\ 
 % \hline
 % \hline
 %     {DPR+PiCL}& ERNIE$_{\text{base}}$&127+128&BM25&49.5&69.36&80.06&86.23\\
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&DPR&\textbf{52.57}&\textbf{71.10}&\textbf{80.50}&\underline{86.84}&-&-&-&-\\ 
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      iiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiii
%\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47 &- &29.78&56.15& 74.20&84.40&34.71&58.79&72.44&81.15\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&31.19&59.2&75.98&85.4\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&32.08&59.56&76.54&85.73& 39.04 & 62.53 & 74.93 & 82.74 \\
     %%%%%% 
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &34.76 &59.72 &74.76 &83.57\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &44.74&66.81&79.31&85.65&53.83&70.34&79.06&84.51\\
     %%%%%% 
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & DPR &52.19&71.19&80.36&86.64& - &- & - & - \\
     % DPR$^*$  &BERT$_{\text{base}}$& 47+48&DPR&\\
     
%\hline 


     % {DPR+PiCL}&BERT$_{\text{base}}$& 47&-& 29.47 & {56.79} & 74.93 & 84.57&35.81&59.54&72.26&81.11\\
     % {DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random& 44.85 & {68.01} & {78.78} & {85.71}\\ 
     %%%%%% Uncommment this
     %{DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random&33.99&61.88&77.7&85.84& - &- & - & - \\
     %%%%%%
     % {DPR+PiCL} & 15+16(R) 	& 59.39	& 76.64	& 86.04   & - & -  \\ 
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&{45.38}&66.79&78.53&85.04& 54.49 & 70.27 & 78.71 & 84.73\\ 
     %%%%%%
     % {DPR+PiCL} & 15+16(BM25)	& - &62.77	&78.06	&\textbf{86.15}  && \\
     % \hline
     % \hline
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&DPR&{52.40}&{70.69}&{80.06}&{86.34}& - &- & - & - \\ 
     %%%%%% 
     % \textbf{ANCE+PiCL} &15+16 & -  & \textbf{-} & \textbf{-}   & - & - \\ 
%\hline
 \noalign{\hrule height 0.8pt}

%     \multicolumn{4}{c}{}&\multicolumn{4}{c}{\textbf{Trivia QA}}\\
% \hline
% \noalign{\hrule height 0.8pt}
%     DPR$^*$ &BERT$_{\text{base}}$& 47 &- &34.71&58.79&72.44&81.15\\
%     DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &53.83&70.34&79.06&84.51\\
% \hline
%     {DPR+PiCL}&BERT$_{\text{base}}$& 47&-&35.81&59.54&72.26&81.11\\
%     {DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&\\
% \hline
 \end{tabular}
\caption{Main results on Natural Questions and TriviaQA benchmark. The best and second results from DPR based retrievers are in \textbf{Bold} and \underline{underline}, respectively. PLMs: pre-trained LMs used for retriever initialization, \#N: the number of negative samples, computed as in-batch negatives + hard negatives, $^*$ denotes reproduced results in our environment setting where \#N=127+128. $^\dag$ indicates reported results from \citet{qu2021rocketqa}. 
% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.
}
\label{table:mainResult}
\end{table*}

==> tables/main_result.tex <==
\begin{table*}[t]\tiny
%\begin{table}
\renewcommand{\arraystretch}{1.2} %1.15
\centering


% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.

\begin{tabular}{l c c c| c c c c| c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{4}{c}{\textbf{Natural Questions}}&\multicolumn{4}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-8}\cmidrule{9-12}
     &PLM &\# Neg (\# IB + \# HN + \# CF)&Hard Neg&R@1 & R@5 &R@20 & R@100&R@1 & R@5 &R@20 & R@100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 59.1 & 73.7 & - & - & 66.9 & 76.7\\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127 & - & - & 55.8 & 73.0 & 83.1 & - & - & 79.4 & 85.0\\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 81.9 & 87.5& - & - & 80.3 & 85.3\\
     RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0& - & - & - & -\\
     RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5& - & - & - & -\\
     %coCondenser$^\dag$&BERT$_{\text{base}}$&-&-&-&75.8&84.3&89.0\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &31.77&58.12&74.76&84.07&38.72&62.56&74.71&82.29\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &46.62&68.56&79.70&86.34&54.26&71.53&79.66&85.34\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+256 & BM25 &45.48&68.25&79.41&86.20&-&-&-&-\\
     DPR$^*$&BERT$_{\text{base}}$&127+128&DPR&52.69& 72.63&81.44&87.48\\
     
% \hline 
 
%      {DPR+SimCCL}&BERT$_{\text{base}}$& 127&-&32.69&60.39&76.73&85.48&43.02&64.05&74.67&82.24\\ 
%      {DPR+SimCCL} &BERT$_{\text{base}}$& 127+128&BM25&\textbf{47.81}&\textbf{69.25}&\textbf{79.92}&\textbf{87.12}&\textbf{56.93}&\textbf{72.32}&\textbf{80.46}&\textbf{85.72}\\ 

%      {DPR+SimCCL} &BERT$_{\text{base}}$& 127+128&DPR&\textbf{52.57}&\textbf{71.10}&\textbf{80.50}&\textbf{86.84}&55.36&70.79&78.46&84.06\\ 
 \hline 
 
     {\our}&BERT$_{\text{base}}$&127+0+128&-&35.35	&61.55	&76.81	&85.87&43.02&64.05&74.67&82.24\\ 
     {\our} &BERT$_{\text{base}}$& 127+128+128&BM25&{48.64}&{69.75}&{80.11}&{86.81}&\textbf{56.93}&\textbf{72.32}&\textbf{80.46}&\textbf{85.72}\\ 
     {\our} &BERT$_{\text{base}}$& 127+128+128&\our&\textbf{54.04}&\textbf{73.88}&\textbf{82.55}&\textbf{87.70}&-&-&-&-\\ 
\hline                                        

\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{Main results on Natural Questions {and TriviaQA benchmarks}. The best results {of DPR based retrievers} are in \textbf{bold}. PLMs {denotes} pre-trained LMs used for retriever initialization, \#N {denotes} the number of negative samples, computed as in-batch negatives + hard negatives, {and }$^*$ denotes reproduced results in our environment setting where \#N=127+128. $^\dag$ indicates reported results from \citet{qu2021rocketqa}.} 

\label{table:mainResult}
\end{table*}

==> tables/main_result_backup.tex <==
\begin{table*}[t]\small
%\begin{table}
\renewcommand{\arraystretch}{1.15} %1.15
\centering

 
\begin{tabular}{l c c c| c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{4}{c}{\textbf{Natural Questions}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-8}
     &PLM &\#N&Hard Neg&Top-1 & Top-5 &Top-20 & Top-100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 59.1 & 73.7 \\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127 & - & - & 55.8 & 73.0 & 83.1 \\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 81.9 & 87.5\\
     RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0\\
     RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5\\
     %coCondenser$^\dag$&BERT$_{\text{base}}$&-&-&-&75.8&84.3&89.0\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &31.77&58.12&74.76&84.07\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &46.62&68.56&79.70&86.34\\
     %DPR$^*$&BERT$_{\text{base}}$&127+128&DPR&52.69& 72.63&81.44&87.48\\
     
\hline 
 
     {DPR+PiCL}&BERT$_{\text{base}}$& 127&-&35.35&61.55&76.81&85.87\\ 
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&BM25&\underline{47.81}&\underline{69.25}&\underline{79.92}&\textbf{87.12}\\ 
 % \hline
 % \hline
 %     {DPR+PiCL}& ERNIE$_{\text{base}}$&127+128&BM25&49.5&69.36&80.06&86.23\\
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&DPR&\textbf{52.57}&\textbf{71.10}&\textbf{80.50}&\underline{86.84}\\ 
%\hline    
%\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47 &- &29.78&56.15& 74.20&84.40&34.71&58.79&72.44&81.15\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&31.19&59.2&75.98&85.4\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&32.08&59.56&76.54&85.73& 39.04 & 62.53 & 74.93 & 82.74 \\
     %%%%%% 
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &34.76 &59.72 &74.76 &83.57\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &44.74&66.81&79.31&85.65&53.83&70.34&79.06&84.51\\
     %%%%%% 
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & DPR &52.19&71.19&80.36&86.64& - &- & - & - \\
     % DPR$^*$  &BERT$_{\text{base}}$& 47+48&DPR&\\
     
%\hline 


     % {DPR+PiCL}&BERT$_{\text{base}}$& 47&-& 29.47 & {56.79} & 74.93 & 84.57&35.81&59.54&72.26&81.11\\
     % {DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random& 44.85 & {68.01} & {78.78} & {85.71}\\ 
     %%%%%% Uncommment this
     %{DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random&33.99&61.88&77.7&85.84& - &- & - & - \\
     %%%%%%
     % {DPR+PiCL} & 15+16(R) 	& 59.39	& 76.64	& 86.04   & - & -  \\ 
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&{45.38}&66.79&78.53&85.04& 54.49 & 70.27 & 78.71 & 84.73\\ 
     %%%%%%
     % {DPR+PiCL} & 15+16(BM25)	& - &62.77	&78.06	&\textbf{86.15}  && \\
     % \hline
     % \hline
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&DPR&{52.40}&{70.69}&{80.06}&{86.34}& - &- & - & - \\ 
     %%%%%% 
     % \textbf{ANCE+PiCL} &15+16 & -  & \textbf{-} & \textbf{-}   & - & - \\ 
%\hline
 \noalign{\hrule height 0.8pt}

%     \multicolumn{4}{c}{}&\multicolumn{4}{c}{\textbf{Trivia QA}}\\
% \hline
% \noalign{\hrule height 0.8pt}
%     DPR$^*$ &BERT$_{\text{base}}$& 47 &- &34.71&58.79&72.44&81.15\\
%     DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &53.83&70.34&79.06&84.51\\
% \hline
%     {DPR+PiCL}&BERT$_{\text{base}}$& 47&-&35.81&59.54&72.26&81.11\\
%     {DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&\\
% \hline
 \end{tabular}
\caption{Main results on Natural Questions benchmark. The best and second results are in \textbf{Bold} and \underline{underline}, respectively. PLMs: pre-trained LMs used for retriever initialization, \#N: the number of negative samples, computed as in-batch negatives + hard negatives, $^*$ denotes reproduced results in our environment setting where \#N=127+128. $^\dag$ indicates reported results from \citet{qu2021rocketqa}. 
% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.
}
\label{table:mainResult}
\end{table*}

==> tables/main_result_backup_new.tex <==
\begin{table*}[t]\small
%\begin{table}
% \renewcommand{\arraystretch}{1.5} %1.15
\centering

 \caption{Main results on Natural Questions \dahyun{and TriviaQA benchmarks}. The best and second results \dahyun{of DPR based retrievers} are in \textbf{Bold} and \underline{underline}, respectively. PLMs: pre-trained LMs used for retriever initialization, \#N: the number of negative samples, computed as in-batch negatives + hard negatives, $^*$ denotes reproduced results in our environment setting where \#N=127+128. $^\dag$ indicates reported results from \citet{qu2021rocketqa}. 
% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.
}
\begin{tabular}{l c c c| c c c c| c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{4}{c}{\textbf{Natural Questions}}&\multicolumn{4}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-8}\cmidrule{9-12}
     &PLM &\#N&Hard Neg&Top-1 & Top-5 &Top-20 & Top-100&Top-1 & Top-5 &Top-20 & Top-100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 59.1 & 73.7 & - & - & 66.9 & 76.7\\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127 & - & - & 55.8 & 73.0 & 83.1 & - & - & 79.4 & 85.0\\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 81.9 & 87.5& - & - & 80.3 & 85.3\\
     RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0& - & - & - & -\\
     RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5& - & - & - & -\\
     %coCondenser$^\dag$&BERT$_{\text{base}}$&-&-&-&75.8&84.3&89.0\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &31.77&58.12&74.76&84.07&38.72&62.56&74.71&82.29\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &46.62&68.56&79.70&86.34&54.26&71.53&79.66&85.34\\
     %DPR$^*$&BERT$_{\text{base}}$&127+128&DPR&52.69& 72.63&81.44&87.48\\
     
\hline 
 
     {DPR+PiCL}&BERT$_{\text{base}}$& 127&-&32.69&60.39&76.73&85.48&43.02&64.05&74.67&82.24\\ 
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&BM25&\underline{47.81}&\underline{69.25}&\underline{79.92}&\textbf{87.12}&\textbf{56.93}&\textbf{72.32}&\textbf{80.46}&\textbf{85.72}\\ 
 % \hline
 % \hline
 %     {DPR+PiCL}& ERNIE$_{\text{base}}$&127+128&BM25&49.5&69.36&80.06&86.23\\
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&DPR&\textbf{52.57}&\textbf{71.10}&\textbf{80.50}&\underline{86.84}&55.36&70.79&78.46&84.06\\ 
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      iiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiii
%\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47 &- &29.78&56.15& 74.20&84.40&34.71&58.79&72.44&81.15\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&31.19&59.2&75.98&85.4\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&32.08&59.56&76.54&85.73& 39.04 & 62.53 & 74.93 & 82.74 \\
     %%%%%% 
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &34.76 &59.72 &74.76 &83.57\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &44.74&66.81&79.31&85.65&53.83&70.34&79.06&84.51\\
     %%%%%% 
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & DPR &52.19&71.19&80.36&86.64& - &- & - & - \\
     % DPR$^*$  &BERT$_{\text{base}}$& 47+48&DPR&\\
     
%\hline 


     % {DPR+PiCL}&BERT$_{\text{base}}$& 47&-& 29.47 & {56.79} & 74.93 & 84.57&35.81&59.54&72.26&81.11\\
     % {DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random& 44.85 & {68.01} & {78.78} & {85.71}\\ 
     %%%%%% Uncommment this
     %{DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random&33.99&61.88&77.7&85.84& - &- & - & - \\
     %%%%%%
     % {DPR+PiCL} & 15+16(R) 	& 59.39	& 76.64	& 86.04   & - & -  \\ 
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&{45.38}&66.79&78.53&85.04& 54.49 & 70.27 & 78.71 & 84.73\\ 
     %%%%%%
     % {DPR+PiCL} & 15+16(BM25)	& - &62.77	&78.06	&\textbf{86.15}  && \\
     % \hline
     % \hline
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&DPR&{52.40}&{70.69}&{80.06}&{86.34}& - &- & - & - \\ 
     %%%%%% 
     % \textbf{ANCE+PiCL} &15+16 & -  & \textbf{-} & \textbf{-}   & - & - \\ 
%\hline
 \noalign{\hrule height 0.8pt}

%     \multicolumn{4}{c}{}&\multicolumn{4}{c}{\textbf{Trivia QA}}\\
% \hline
% \noalign{\hrule height 0.8pt}
%     DPR$^*$ &BERT$_{\text{base}}$& 47 &- &34.71&58.79&72.44&81.15\\
%     DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &53.83&70.34&79.06&84.51\\
% \hline
%     {DPR+PiCL}&BERT$_{\text{base}}$& 47&-&35.81&59.54&72.26&81.11\\
%     {DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&\\
% \hline
 \end{tabular}

\label{table:mainResult}
\end{table*}

==> tables/main_result_full_backup.tex <==
\begin{table*}[t]\small
%\begin{table}
%\renewcommand{\arraystretch}{1.5} %1.15
\centering

 
\begin{tabular}{l c c c| c c c c| c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{4}{c}{\textbf{Natural Questions}}&\multicolumn{5}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-8}\cmidrule{9-13}
     &PLM &\#N&Hard Neg&Top-1 & Top-5 &Top-20 & Top-100&Top-1 & Top-5 &Top-20 & Top-100&MAP@100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 59.1 & 73.7 & - & - & 66.9 & 76.7\\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127 & - & - & 55.8 & 73.0 & 83.1 & - & - & 79.4 & 85.0\\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 81.9 & 87.5& - & - & 80.3 & 85.3\\
     RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0& - & - & - & 86.0\\
     RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5& - & 74.0 & 82.7 & 88.5\\
     %coCondenser$^\dag$&BERT$_{\text{base}}$&-&-&-&75.8&84.3&89.0\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &31.77&58.12&74.76&84.07&38.72&62.56&74.71&82.29\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &46.62&68.56&79.70&86.34&54.26&71.53&79.66&85.34\\
     %DPR$^*$&BERT$_{\text{base}}$&127+128&DPR&52.69& 72.63&81.44&87.48\\
     
\hline 
 
     {DPR+PiCL}&BERT$_{\text{base}}$& 127&-&32.69&60.39&76.73&85.48&43.02&64.05&74.67&82.24\\ 
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&BM25&\underline{47.81}&\underline{69.25}&\underline{79.92}&\textbf{87.12}&\underline{56.93}&\underline{72.32}&\underline{80.46}&\textbf{85.72}\\ 
 % \hline
 % \hline
 %     {DPR+PiCL}& ERNIE$_{\text{base}}$&127+128&BM25&49.5&69.36&80.06&86.23\\
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&DPR&\textbf{52.57}&\textbf{71.10}&\textbf{80.50}&\underline{86.84}&-&-&-&-\\ 
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      iiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiiii
%\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47 &- &29.78&56.15& 74.20&84.40&34.71&58.79&72.44&81.15\\
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&31.19&59.2&75.98&85.4\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & random&32.08&59.56&76.54&85.73& 39.04 & 62.53 & 74.93 & 82.74 \\
     %%%%%% 
     % DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &34.76 &59.72 &74.76 &83.57\\
     %%%%%% Uncommment this
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &44.74&66.81&79.31&85.65&53.83&70.34&79.06&84.51\\
     %%%%%% 
     %DPR$^*$ &BERT$_{\text{base}}$& 47+48 & DPR &52.19&71.19&80.36&86.64& - &- & - & - \\
     % DPR$^*$  &BERT$_{\text{base}}$& 47+48&DPR&\\
     
%\hline 


     % {DPR+PiCL}&BERT$_{\text{base}}$& 47&-& 29.47 & {56.79} & 74.93 & 84.57&35.81&59.54&72.26&81.11\\
     % {DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random& 44.85 & {68.01} & {78.78} & {85.71}\\ 
     %%%%%% Uncommment this
     %{DPR+PiCL}&BERT$_{\text{base}}$& 47+48&random&33.99&61.88&77.7&85.84& - &- & - & - \\
     %%%%%%
     % {DPR+PiCL} & 15+16(R) 	& 59.39	& 76.64	& 86.04   & - & -  \\ 
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&{45.38}&66.79&78.53&85.04& 54.49 & 70.27 & 78.71 & 84.73\\ 
     %%%%%%
     % {DPR+PiCL} & 15+16(BM25)	& - &62.77	&78.06	&\textbf{86.15}  && \\
     % \hline
     % \hline
     %%%%%% Uncommment this
     %{DPR+PiCL} &BERT$_{\text{base}}$& 47+48&DPR&{52.40}&{70.69}&{80.06}&{86.34}& - &- & - & - \\ 
     %%%%%% 
     % \textbf{ANCE+PiCL} &15+16 & -  & \textbf{-} & \textbf{-}   & - & - \\ 
%\hline
 \noalign{\hrule height 0.8pt}

%     \multicolumn{4}{c}{}&\multicolumn{4}{c}{\textbf{Trivia QA}}\\
% \hline
% \noalign{\hrule height 0.8pt}
%     DPR$^*$ &BERT$_{\text{base}}$& 47 &- &34.71&58.79&72.44&81.15\\
%     DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &53.83&70.34&79.06&84.51\\
% \hline
%     {DPR+PiCL}&BERT$_{\text{base}}$& 47&-&35.81&59.54&72.26&81.11\\
%     {DPR+PiCL} &BERT$_{\text{base}}$& 47+48&BM25&\\
% \hline
 \end{tabular}
\caption{Main results on Natural Questions and TriviaQA benchmark. The best and second results from DPR based retrievers are in \textbf{Bold} and \underline{underline}, respectively. PLMs: pre-trained LMs used for retriever initialization, \#N: the number of negative samples, computed as in-batch negatives + hard negatives, $^*$ denotes reproduced results in our environment setting where \#N=127+128. $^\dag$ indicates reported results from \citet{qu2021rocketqa}. 
% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.
}
\label{table:mainResult}
\end{table*}

==> tables/main_result_ndcg.tex <==
\begin{table*}[t]\tiny
%\begin{table}
\renewcommand{\arraystretch}{1.2} %1.15
\centering


% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.

\begin{tabular}{l | c c c c c c| c c c c c c }
 \hline
 \noalign{\hrule height 0.8pt}
  {\textbf{Retriever}}&\multicolumn{6}{c}{\textbf{Natural Questions}}&\multicolumn{6}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-7}\cmidrule{8-13}
      ~~~+ \#N Hard Neg &Top-1&Top-20 &Top-100&MAP@10&MRR@10&nDCG@10&Top-1&Top-20 &Top-100&MAP@10&MRR@10&nDCG@10
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & 59.1 & 73.7 & - & - & - & - & 66.9 & 76.7& -& - & - \\ 
     DPR$^\dag$ & - & 73.0 & 83.1 & - & - & - & - & 79.4 & 85.0 & - & - & - \\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & - & 81.9 & 87.5& - & - & - & - & 80.3 & 85.3& - & - & - \\
     RocketQA$_{\text{step1}}^\dag$ & - & - & 86.0 & - & - & - & - & - & - & - & - & - \\
     RocketQA$^\dag$ & - & 82.7 & 88.5& - & - & -  & - & -& - & - & - & - \\
     %coCondenser$^\dag$&BERT$_{\text{base}}$&-&-&-&75.8&84.3&89.0\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$&31.77&74.76&84.07& 23.77 & 43.14 &47.81&38.72&74.71&82.29&31.50 &49.30 &52.22\\
     ~~~+ 1 BM25 Neg &46.62&79.70&86.34& 30.86 & 56.01 &58.36&54.26&79.66 &85.34 &43.29 &62.03 & 63.05\\
     ~~~+ 2 BM25 Neg &45.48 &79.41 &86.20 &30.34 &55.03 &57.85&54.70&80.19&85.59&45.15&62.30&64.58\\
     ~~~+ 1 DPR Neg&52.69& 81.44&87.48 &35.37 &61.17&62.81&54.19&78.22&84.27&41.36&61.25&61.91\\
     DPR$_{\texttt{condenser}}$&27.87&73.10&84.63&22.85&39.22&44.31&37.73&74.80&82.96&32.16&48.70&51.99\\
~~~+ 1 BM25 Neg &48.61 &80.72 &86.68&31.98 &57.79 &59.69 & 57.70 & \textbf{81.32} & \textbf{86.27} & \textbf{49.83} & \textbf{64.96} & \textbf{66.29} \\
\hline    
 
     {\our}&35.35 &76.81&85.87& 25.77 &46.41  &50.87&43.02&74.67&82.24 &34.10 &52.42 &54.53\\ 
     
     % {\our}&35.35 &76.81&85.87& - &46.41  &52.08&43.02&74.67&82.24\\ 

     
     ~~~+ 1 BM25 Neg&{48.64}&{80.11}
&{86.81}& 32.89 & 57.58 &59.65&56.93&80.46&85.72&45.15 &63.92&64.58 \\ 
     ~~~+ 1 \our~Neg&\textbf{54.04}&\textbf{82.55}&\textbf{87.70}&\textbf{36.41}&\textbf{62.37}&\textbf{63.71}&54.12&77.95&83.71 &41.58 &61.19 & 61.74\\    
% \our $_{\texttt{ERNIE}}$&&&&&&&&&&&&\\
% ~~~+ 1 \our~Neg &54.84 &82.66 &87.59 &- &- &- &- &- &- &- &- &- \\
\our $_{\texttt{condenser}}$&34.10&77.23&85.15&25.31&45.89&50.51&39.26&75.29&82.62&32.20&50.15&53.33\\
~~~+ 1 BM25 Neg &50.06 &80.80 &86.81 &32.58 &59.14 &60.93 & \textbf{57.98} & 80.73 &85.69 & 45.43 & 64.75 & 65.26 \\

\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{Main results on Natural Questions {and TriviaQA benchmarks}. Top-$k$ hit accuracy, MAP, MRR, and nDCG scores are reported. The best results {of DPR-based retrievers} are in \textbf{bold}. DPR and AADPR use in-batch training, and ``+ \#N Hard Neg'' denotes a \#N number of additional negatives obtained by the aligned  retriever. $^*$ denotes reproduced results in our environment setting, and $^\dag$ indicates reported results from \citet{qu2021rocketqa}.} 

\label{table:mainResult_old}
\end{table*}

==> tables/main_result_new.tex <==
\begin{table*}[t]\small
%\begin{table}
%\renewcommand{\arraystretch}{1.5} %1.15
\centering

 
\begin{tabular}{l c c c| c c c c| c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{4}{c}{\textbf{Natural Questions}}&\multicolumn{4}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-8}\cmidrule{9-12}
     &PLM &\#N&Hard Neg&Top-1 & Top-5 &Top-20 & Top-100&Top-1 & Top-5 &Top-20 & Top-100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 59.1 & 73.7 & - & - & 59.1 & 73.7\\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127 & - & - & 55.8 & 73.0 & 83.1 & - & 55.8 & 73.0 & 83.1\\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 81.9 & 87.5& - & - & 81.9 & 87.5\\
     RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0& - & - & - & 86.0\\
     RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5& - & 74.0 & 82.7 & 88.5\\

\hline
\hline
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &31.77&58.12&74.76&84.07&38.72&62.56&74.71&82.29\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &46.62&68.56&79.70&86.34&54.26&71.53&79.66&85.34\\
\hline 
 
     {DPR+PiCL}&BERT$_{\text{base}}$& 127&-&32.69&60.39&76.73&85.48&43.02&64.05&74.67&82.24\\ 
     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&BM25&\underline{47.81}&\underline{69.25}&\underline{79.92}&\textbf{87.12}&\underline{56.93}&\underline{72.32}&\underline{80.46}&\textbf{85.72}\\ 

     {DPR+PiCL} &BERT$_{\text{base}}$& 127+128&DPR&\textbf{52.57}&\textbf{71.10}&\textbf{80.50}&\underline{86.84}&-&-&-&-\\ 

 \noalign{\hrule height 0.8pt}
 \end{tabular}
\caption{Main results on Natural Questions benchmark. The best and second results are in \textbf{Bold} and \underline{underline}, respectively. PLMs: pre-trained LMs used for retriever initialization, \#N: the number of negative samples, computed as in-batch negatives + hard negatives, $^*$ denotes reproduced results in our environment setting where \#N=127+128. $^\dag$ indicates reported results from \citet{qu2021rocketqa}. 

}
\label{table:mainResultFull}
\end{table*}

==> tables/main_result_trivia.tex <==
\begin{table*}[t]\small
%\begin{table}
\renewcommand{\arraystretch}{1.3} %1.15
\centering

 
\begin{tabular}{l c c c| c c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
  \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{3}{c}{\textbf{Training Resource}}&\multicolumn{5}{c}{\textbf{TriviaQA}}
  \\ 
  \cmidrule(lr){2-4}\cmidrule(lr){5-9}
     &PLM &\#N&Hard Neg&Top-1 &Top-5 &Top-20 &Top-100 & MAP@100
     \\
 
\hline

\noalign{\hrule height0.8pt}
     BM25$^\dag$ & - & - &- & - & - & 66.9 & 76.7 & - \\ 
     DPR$^\dag$ &BERT$_{\text{base}}$ & 127+128 & BM25 & - & - & 79.4 & 85.0 & -\\
     % DPR$^\dag$ &ERNIE$_{\text{base}}$ & 127 & - & - & 68.4&80.7&87.3 \\
     ANCE$^\dag$ & RoBERTa$_{\text{base}}$ & 31+32 & ANN& - & - & 80.3 & 85.3 & -\\
     %RocketQA$_{\text{step1}}^\dag$ &BERT$_{\text{base}}$&1023+1024&Cross Batch& - & - & - & 86.0\\
     %RocketQA$^\dag$ &ERNIE$_{\text{base}}$&1023+1024&Cross Encoder& - & 74.0 & 82.7 & 88.5\\

% 128 reproduce setting
\hline
\hline
     % DPR$^*$ & 47 &- & 29.78 & 56.15  & 68.39 & 81.25\\
     DPR$^*$ &BERT$_{\text{base}}$& 127 &- &38.72&62.56&74.71&82.29 & 27.78\\
     DPR$^*$ &BERT$_{\text{base}}$& 127+128 & BM25 &54.26&71.53&79.66&85.34 & 31.36\\
     %DPR$^*$&BERT$_{\text{base}}$&127+128&DPR&52.69& 72.63&81.44&87.48\\
     
\hline 
 
     {\our}&BERT$_{\text{base}}$& 127&-&43.02&64.05&74.67&82.24& 37.93\\ 
     {\our} &BERT$_{\text{base}}$& 127+128&BM25&\textbf{56.93}&\textbf{72.32}&\textbf{80.46}&\textbf{85.72} & \textbf{39.4}\\ 

 \noalign{\hrule height 0.8pt}

%     \multicolumn{4}{c}{}&\multicolumn{4}{c}{\textbf{Trivia QA}}\\
% \hline
% \noalign{\hrule height 0.8pt}
%     DPR$^*$ &BERT$_{\text{base}}$& 47 &- &34.71&58.79&72.44&81.15\\
%     DPR$^*$ &BERT$_{\text{base}}$& 47+48 & BM25 &53.83&70.34&79.06&84.51\\
% \hline
%     {\our}&BERT$_{\text{base}}$& 47&-&35.81&59.54&72.26&81.11\\
%     {\our} &BERT$_{\text{base}}$& 47+48&BM25&\\
% \hline
 \end{tabular}
\caption{Retrieval results on TriviaQA benchmark, reported by R@$k$ accuracies and MAP. The best results are in \textbf{Bold}. PLMs: pre-trained LMs used for retriever initialization, \#N: the number of negative samples, computed as in-batch negatives + hard negatives, $^*$ denotes reproduced results in our setting where \#N=127+128. $^\dag$ indicates reported results from prior work~\citep{karpukhin2020dpr,xiong2020ance,qu2021rocketqa}. 
}
\label{table:mainResultTrivia}
\end{table*}


==> tables/model-compare-new.tex <==
\begin{table*}[t]\small
%\begin{table}
%\renewcommand{\arraystretch}{1.5} %1.15

\centering
\begin{tabular}{l c c c c l l}
 \hline
 \noalign{\hrule height 0.8pt}
    Retriever & Min.GPU & PLM & Batch Size & Iterative Sampling & Index Refresh & KD Teacher \\
    % \multirow{2}{*}{\textbf{Training}}&\multicolumn{3}{c}{\textbf{NaturalQuestions}}\\
    % &top-1 &top-20 & top-100 \\
\hline
\noalign{\hrule height0.8pt}
     DPR / DPR+PiCL &1$\times$GTX & BERT & 32 & - & - & - \\
     ANCE & \textbf{4$\times$V100} & RoBERTa & 32 & \cmark & \textbf{Per 10K batches} & - \\
     RocketQA$_\text{step1}$& 2$\times$V100 & BERT & \textbf{1024} & - & - & - \\
     RocketQA& 2$\times$V100 & ERNIE & \textbf{1024} & \cmark & 2$\times$ & \textbf{Cross Encoder} \\
     
\hline
\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{Comparison of the required resource for various dense retrieval approaches.}
%Each column indicates minimal GPU resources to train, reported batch size, whether using knowledge distillation teacher, and the frequency of refresh indices (passage resampling) during training, respectively, reported on \citep{hofstatter2021efficiently}.}
\label{table:model-compare}
\end{table*}

==> tables/more_metrics.tex <==
\begin{table}[t]\small

\renewcommand{\arraystretch}{1.2} %1.15

\begin{subtable}[h]{\linewidth}
  \centering
  \begin{tabular}{l | c c c}
    \hline
    \noalign{\hrule height 0.8pt}
    \textbf{ Retriever}&\multicolumn{3}{c}{\textbf{Natural Questions}}\\
    \cmidrule(lr){2-4}
    (+Hard Neg)&MAP@100 & MRR@10 & nDCG@10\\
    \hline
    \noalign{\hrule height0.8pt}
     DPR$^*$ &&43.85&47.81\\
     ~~~~~+BM25&&56.50&58.46\\
     ~~~~~+DPR\\
    \hline 
     \our&&48.88&52.08\\
     ~~~~~+BM25&&57.49&59.27\\
     ~~~~~+\our\\
     \hline
     \noalign{\hrule height0.8pt}
  \end{tabular}
  \caption{Performance comparison on Natural Questions}
  \label{table:more-metrics-NQ}
\end{subtable}
\hfill
\\
\\
\begin{subtable}[h]{\linewidth}
    \begin{tabular}{l | c c c}
    \hline
    \noalign{\hrule height 0.8pt}
    \textbf{ Retriever}&\multicolumn{3}{c}{\textbf{TriviaQA}}\\ 
    \cmidrule(lr){2-4}
    (+Hard Neg)&MAP@100 & MRR@10 & nDCG@10\\
    \hline
    \noalign{\hrule height0.8pt}
% 128 reproduce setting
    DPR$^*$ &27.78\\
     ~~~~~+BM25&31.36\\
     ~~~~~+DPR\\
    \hline 
    \our&37.93\\
     ~~~~~+BM25&39.4\\
     ~~~~~+\our\\
    \hline
    \noalign{\hrule height 0.8pt}
    \end{tabular}
    \caption{Performance comparison on TriviaQA}
\label{table:more-metrics-TQA}
\end{subtable}
\caption{Retrieval performances with more precise metrics (\eg, MAP, MRR, and nDCG). The best results are in \textbf{bold}.} 
\label{table:more-metrics}
\end{table}

==> tables/parameters.tex <==
\begin{table*}[!ht]\small

\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l c c c | c c c c}
 \hline
 \noalign{\hrule height 0.8pt}
    \multirow{2}{*}{\textbf{Retriever}}&\multicolumn{3}{c}{\textbf{Loss}}&\multicolumn{4}{c}{\textbf{NaturalQuestions}}\\
    &$\mathcal{L}_{\texttt{dpr}}$&$\mathcal{L}_{\texttt{chn}}$&$\mathcal{L}_{\texttt{cpp}}$&top-1&top-5&top-20 & top-100 \\
\hline
\noalign{\hrule height0.8pt}
DPR &&&&29.78&56.15&74.2&84.4 \\
\hline
     \multirow{4}{*}{PiCL} & 1& 0.1&0.1&&&& \\
     &1&0.2&0.2&29.92&57.09&75.26&84.46\\
     &1&1&1&29.14&57.81&74.6&84.4\\
     &1&2&1&28.64&57.65&75.15&84.1 \\
     
     
     
\hline
 \noalign{\hrule height 0.8pt}
 \end{tabular}
 
\caption{} 
\label{table:parameters}

\end{table*}




==> tables/qtype_example.tex <==
\begin{table}[h]\small
\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{l c  l c}
\hline
\noalign{\hrule height 0.8pt}
     \textbf{Question: } & \multicolumn{3}{c}{
        who died in the plane crash greys anatomy
     } \\
     \textbf{Answer: } & \multicolumn{3}{c}{
        
     } \\
     \textbf{Answer Passage: } & \multicolumn{3}{c}{
        ''Flight'' is the twenty-fourth and final episode of the eighth season of the American television medical drama Grey 's Anatomy … six doctors from Seattle Grace Mercy West Hospital who are victims of an aviation accident fight to stay alive , but Dr. Lexie Grey ( Chyler Leigh ) ultimately dies . … 
     } \\
     
\noalign{\hrule height 0.8pt}
    \multicolumn{2}{c}{\textbf{DPR}}&\multicolumn{2}{c}{\textbf{DPR+PiCL}}\\
    Top-1 Passage &  &
    Top-1 Passage & \\
    Top- Passage &  &
    Top- Passage & \\
\hline
\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{An example case of DPR failure on "who" questions.}
\label{tab:qtype_example}
\end{table}

==> tables/robustness.tex <==
\begin{table*}[t]\small
% \begin{table}
\renewcommand{\arraystretch}{1.5} %1.15
\centering
\caption{Robustness on perturbed dataset.
The best result is in \textbf{Bold}. 
$^\dag$ denotes checkpoints provided by \citet{karpukhin2020dpr} \citet{xiong2020ance}, and \citet{qu2021rocketqa}. 
} 
\begin{tabular}{l c c | c c}
 \hline
 \noalign{\hrule height 0.8pt}
 \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{2}{c}{\textbf{NaturalQuestions}}&\multicolumn{2}{c}{\textbf{Perturbed NaturalQuestions}} \\
     &top-20 & top-100 & top-20 & top-100 \\
\hline


\noalign{\hrule height0.8pt}
     DPR$^\dag$ & 68.39 & 81.25  & - & - \\
     % ANCE$^\dag$ & - & -  & - & - \\ 
     RocketQA$^\dag$ &82.7 &88.5  & - & - \\
     {DPR+PiCL} {78.78} & {85.71}  & - & -  \\ 
     % \textbf{ANCE+PiCL} & - & -  & - & - \\ 
\hline

 \noalign{\hrule height 0.8pt}
 \end{tabular}
 

\label{table:robustness}
\end{table*}
% \end{table}



==> tables/robustness_adversarial.tex <==
\begin{table}[h]\small
% \begin{table}
\renewcommand{\arraystretch}{1.5} %1.15
\centering
\begin{tabular}{l c c}
 \hline
 \noalign{\hrule height 0.8pt}
 \multirow{2}{*}{\textbf{ Retriever}}&\multicolumn{2}{c}{\textbf{Perturbed NaturalQuestions}} \\
    &top-20 & top-100 \\
\hline

\noalign{\hrule height0.8pt}
     DPR$^\dag$  & - & - \\
     DPR$_\text{neg}$ & - & - \\
     DPR$_\text{pos}$ & - & - \\
     {DPR+PiCL} & - & -  \\ 
\hline

\noalign{\hrule height 0.8pt}
\end{tabular}
 
\caption{Robustness on perturbed dataset. The best result is in \textbf{Bold}. $^\dag$ denotes checkpoints provided by \citet{karpukhin2020dpr} \citet{xiong2020ance}, and \citet{qu2021rocketqa}. } 

\label{table:robustness_adversarial}
\end{table}
% \end{table}



==> tables/score_diff_table.tex <==
\begin{table}[t]\small
\renewcommand{\arraystretch}{1.15} %1.15
\centering

\begin{tabular}{l c c}
\hline
\noalign{\hrule height 0.8pt}
    Samples & \textbf{DPR} & \textbf{DPR+PiCL} \\
\hline
    Answer-aware & 1.99 & 3.38 \\
    Answer-unaware & -0.98 & -1.12 \\
\hline
    All & 1.12 & 2.85 \\
\hline
\noalign{\hrule height 0.8pt}
\end{tabular}

\caption{Average score differences between $\langle q,p^+ \rangle$ and $\langle q,p^* \rangle$, measured using both DPR and DPR+PiCL. 
Score differences are measured on two sets of $(q,p^+,p^*)$ triplets, one that satisfies $\langle q,p^+ \rangle > \langle q,p^* \rangle$ (\ie{ Answer-aware}) and another that doesn't (\ie{ Answer-unaware}).}

\label{tab:score_diff}
\end{table}

% Average score differences between $sim(q,p^+)$ and $sim(q,p^*)$, measured using both DPR and DPR+PiCL. Score differences are measured on two sets of $(q,p^+,p^*)$ triplets: divided by the definition of Answerability-relevance mismatch from Section~\ref{sec:robustness_analysis}.

==> tables/table_counterfactual_sampling.tex <==
\begin{table}[t]\small
%\begin{table}
\renewcommand{\arraystretch}{1.2} %1.15
\centering


% $_{\text{BM25}}$, and $_{\text{DPR}}$ indicates two hard negative sampling methods : BM25, DPR inference respectively.

\begin{tabular}{l c c c c}
\hline
\noalign{\hrule height 0.8pt}
 & \multicolumn{4}{c}{\textbf{Natural Questions}} \\ 
\cmidrule(lr){2-5}
{\textbf{Strategies}}&Top-1&Top-20 &Top-100 & MRR \\
 
\hline
\hline 
Span masking & 48.64 & 80.11 & 86.81 & 56.50 \\ 
Span replacement & & & & \\
~~~~~via retrieval & 50.13 & 80.02 & 86.32 & 58.84 \\ 
~~~~~via generation & - & - & - & - \\    
\hline
\multicolumn{4}{l}{\textit{Evidentiality Annotation}}\\
Span masking & 48.64 & 80.11 & 86.81 & 56.50 \\ 
Span replacement & & & & \\
~~~~~via retrieval & 50.13 & 80.02 & 86.32 & 58.84 \\ 
~~~~~via generation & - & - & - & - \\

\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{Comparison between different counterfactual sampling strategies.} 

\label{table:counterfactual_sampling}
\end{table}

==> tables/task_taxonomy.tex <==
\begin{table}[t]\small
\renewcommand{\arraystretch}{1.5} %1.15
\centering

\begin{tabular}{c c c}
\hline
\noalign{\hrule height 0.8pt}
     Categories & Tasks & Benchmarks \\ \hline
     
     \multirow{2}{*}{Extractive} & Open-domain QA & NQ, TQA \\ \cline{2-3}
                                 & Slot Filling & T-REx \\
     \hline
     \multirow{2}{*}{Abstractive} & Dialogue & Wizard of Wikipedia \\ \cline{2-3}
                                  & Multi-hop QA & HotpotQA \\
\hline
\noalign{\hrule height 0.8pt}
\end{tabular}
\caption{Taxonomy of target tasks in our paper.}
\label{tab:task_taxonomy}
\end{table}
